Exploring Forgetting in Large Language Model Pre-Training

Catastrophic forgetting remains a formidable obstacle to building an omniscient model in large language models (LLMs). Despite the pioneering research on task-level forgetting in LLM fine-tuning, there is scant focus on forgetting during pre-training. We systematically explored the existence and measurement of forgetting in pre-training, questioning traditional metrics such as perplexity (PPL) and introducing new metrics to better detect entity memory retention. Based on our revised assessment of forgetting metrics, we explored low-cost, straightforward methods to mitigate forgetting during the pre-training phase. Further, we carefully analyzed the learning curves, offering insights into the dynamics of forgetting. Extensive evaluations and analyses on forgetting of pre-training could facilitate future research on LLMs.

==> 2_related_work_bak.tex <==
\section{Related Work}

% TODO
% 先讲lm中的forgetting, 也有task level的forgetting, 讲一些解决方法, 然后说普遍都是回放方法, 缺乏对forgetting现象的探索, 顺便提一下replay

\paragraph{Catastrophic Forgetting in Language Models.} 
Neural networks typically exhibit a phenomenon known as catastrophic forgetting~\citep{mccloskey1989catastrophic, ratcliff1990connectionist} when trained on new tasks, where they tend to lose previously acquired knowledge. This phenomenon is commonly attributed to a shift in the distribution of the input data. A number of mechanisms have been proposed to alleviate forgetting in this setting.~\citet{sun2020ernie} constructed three different kinds of pre-training tasks, and they simultaneously train the newly-introduced task and the original task whenever a new task comes.~\citet{jin2021lifelong} investigated lifelong pre-training by incrementally pre-training a language model using continual learning algorithms on both domain-incremental and chronologically-ordered data streams.~\citet{de2019episodic} explored the integration of episodic memory mechanisms within lifelong learning frameworks to enhance language model training. They demonstrate that this mechanism enables the model to sustain continuous learning from a diverse range of data distributions.~\citet{wang2020efficient} introduced a meta-lifelong framework to mitigate the issue of catastrophic forgetting.~\citet{qin2022elle} introduced function-preserved model expansion to enhance the efficiency of knowledge acquisition by dynamically augmenting the dimensions of a pre-existing PLM. Nonetheless, the majority of these studies have not extensively examined situations characterized by a sole data distribution, while our research delves deeply into the pre-training context where data is exclusively drawn from a single distribution. 



% 这部分讲example forgetting, 和对example forgetting的探索
\paragraph{Example Forgetting and Forgetting During Pre-training.}  Despite the extensive research on catastrophic forgetting, there remains a dearth of investigation into the understanding of data forgetting within what is traditionally considered a single task. Example forgetting was first defined by~\citet{toneva2018empirical}. It was observed that throughout the entire training process of what is usually considered to be a single task, certain examples are correctly classified at some $t$, and then subsequently misclassified.~\citet{tirumala2022memorization} investigated the dynamics of memorization and forgetting in language models. They characterized the forgetting curves and assessed the relationship between the memorization dynamics throughout the training process and the dimensions of the model.~\citet{biderman2023emergent} introduced a novel approach to model behavior forecasting by extrapolating from low-cost training data, allowing for efficient model termination and pioneering the extrapolation from partially trained to fully trained models.~\citet{gupta2023continual} explored the effects of diverse warm-up strategies within the context of continual pre-training, a process that involves the ongoing pre-training of existing models with new data. While these studies have delved into the phenomenon of forgetting during the pre-training phase, none have provided a more nuanced or specific formalization of what is forgotten and how this forgetting is quantified using metrics.

